Synthetic Data Augmentation for Zero-Shot Cross-Lingual Question Answering

Coupled with the availability of large scale datasets, deep learning architectures have enabled rapid progress on the Question Answering task. However, most of those datasets are in English, and the performances of state-of-the-art multilingual models are significantly lower when evaluated on non-English data. Due to high data collection costs, it is not realistic to obtain annotated data for each language one desires to support. We propose a method to improve the Cross-lingual Question Answering performance without requiring additional annotated data, leveraging Question Generation models to produce synthetic samples in a cross-lingual fashion. We show that the proposed method allows to significantly outperform the baselines trained on English data only. We report a new state-of-the-art on four multilingual datasets: MLQA, XQuAD, SQuAD-it and PIAF (fr).

==> Makefile <==
# set latexfile to the name of the main file without the .tex
#latexfile = eacltest
latexfile = emnlp2021

# put the names of figure files here.  include the .eps
figures = 

#includedfiles = Intro.tex State-of-the-art.tex Experiments.tex Discussion.tex
includedfiles = 
#1Discussion.tex Intro_Djame.tex









#Algos.tex Discussion.tex Results.tex \
#	eacltest.tex experiences.tex intro.tex lexical-inpact.tex \
#	presentation-treebank.tex protocol.tex state-of-the-art-comparaison.tex\
#	corpus-setup-experiment.tex TODO.tex Tagset.tex crossparsing.tex \
#	new_intro.tex new_presTB.tex new_protocol.tex examples-marie.tex

TEX = pdflatex

# *.fig files may be in ./Figs
vpath %.fig Figs


all: pdf
$(latexfile).dvi : $(figures) $(includedfiles) $(latexfile).tex


%.eps : %.fig
	fig2dev -L eps $< > $@

$(latexfile).pdf : $(latexfile).tex $(includedfiles) $(figures)
	$(TEX)  $(latexfile).tex
#	$(TEX)  appendix.tex

pdf :	$(latexfile).tex
	$(TEX) $(latexfile).tex 

bib : $(latexfile).tex
	$(TEX) $(latexfile)
	bibtex $(latexfile)
	$(TEX) $(latexfile)
	$(TEX) $(latexfile)
#	bibtex $(latexfile)
#	$(TEX) $(latexfile)
#	$(TEX) $(latexfile)
#	$(TEX) $(latexfile)
	
	 
force:
	$(TEX)  appendix.tex
	bibtex appendix
	$(TEX) appendix
	$(TEX) appendix
	bibtex appendix
	$(TEX) appendix
	$(TEX) appendix

appendix.pdf: 
	$(TEX)  appendix.tex
	bibtex appendix
	$(TEX) appendix
	$(TEX) appendix
	bibtex appendix
	$(TEX) appendix
	$(TEX) appendix

	

$(latexfile).ps : $(latexfile).dvi
	dvips  -Ppdf $(latexfile) -o $(latexfile).ps

ps : $(latexfile).ps 

$(latexfile).tar.gz : $(figures) $(latexfile).tex
	tar -czvf $(latexfile).tar.gz $(figures) $(latexfile).tex Figs/*.fig

tarball: $(latexfile).tar.gz


clean: 
	rm -f $(latexfile).bbl
	rm -f $(latexfile).log
	rm -f $(latexfile).dvi
	rm -f $(latexfile).blg
	rm -f $(latexfile).aux
	rm -f $(latexfile).ps
	rm -f $(latexfile).pdf
	rm -f $(latexfile).out
	
clean2:
	rm -f appendix.bbl
	rm -f appendix.log
	rm -f appendix.dvi
	rm -f appendix.blg
	rm -f appendix.aux
	rm -f appendix.ps
	rm -f appendix.pdf
		
check:
	cat $(latexfile).log | grep --text undef
	cat $(latexfile).log | grep --text multipl

dist-clean: clean
	rm -f $(latexfile).ps
	rm -f $(latexfile).pdf

viewX: pdf 
	open $(latexfile).pdf
	
viewA: pdf
	open -a Preview.app $(latexfile).pdf

view: $(latexfile).pdf
	open -a Skim.app $(latexfile).pdf
#	open -a Skim.app appendix.pdf 

gv: ps
	gv $(latexfile).pdf


edit: 
	xemacs $(latexfile).tex  & 


up:
	git pull

co:	commit
	
commit:
	git commit -m "update" 	./
	git push

commitsvn:
	svn commit -m "update" ./

upsvn:
	svn up

cp:
#	TEMP := $(shell mktemp -u)
	cp $(latexfile).pdf /Users/djame2/Library/Mobile\ Documents/3L68KQB4HG~com~readdle~CommonDocuments/Documents/PapiersEnCours/$(latexfile)_$(shell gdate +%F_%R).pdf

final: pdf 
	cp $(latexfile).pdf ./WNUT2021_CharacterBert4UGC_Riabi_Seddah.pdf
	

ebib:
	open $(latexfile).bib


split: bib
	splitappendix $(latexfile).pdf 12
	open -a Skim.app submission.pdf appendix.pdf
	

